MixTailor: Mixed Gradient Aggregation for Robust Learning Against Tailored Attacks

Implementations of SGD on distributed systems create new vulnerabilities, which can be identified and misused by one or more adversarial agents. Recently, it has been shown that well-known Byzantine-resilient gradient aggregation schemes are indeed vulnerable to informed attackers that can tailor the attacks (Fang et al., 2020; Xie et al., 2020b). We introduce MixTailor, a scheme based on randomization of the aggregation strategies that makes it impossible for the attacker to be fully informed. Deterministic schemes can be integrated into MixTailor on the fly without introducing any additional hyperparameters. Randomization decreases the capability of a powerful adversary to tailor its attacks, while the resulting randomized aggregation scheme is still competitive in terms of performance. For both iid and non-iid settings, we establish almost sure convergence guarantees that are both stronger and more general than those available in the literature. Our empirical studies across various datasets, attacks, and settings, validate our hypothesis and show that MixTailor successfully defends when well-known Byzantine-tolerant schemes fail.

==> sections/fig_cifar_iid.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=.9\linewidth]{figs/cifar10-stochastic-lr-0.001-reverse-0.1-bs-80/Vacc-li.pdf}\\
    % \includegraphics[width=.49\textwidth]{figures/imagenet_last/loss.pdf}
    % \hfill
    \includegraphics[width=.9\linewidth]{figs/cifar10-stochastic-lr-0.001-reverse-10-bs-80/Vacc-li.pdf}
%    \hfill
%    \includegraphics[width=.32\textwidth]{figures/cifar10_gvar/est_nvar.pdf}
    \caption{Test accuracy on CIFAR-10 with $\epsilon=0.1$ (top) and 
    $\epsilon=10$ (bottom) for the tailored attack, which is applied at each iteration.
    The total number of workers and the number of Byzantines are set to  $\nAll=12$ and $\nByz=2$, respectively.
    The dataset is randomly and equally partitioned among workers. 
	The omniscient aggregator receives and averages 10 honest gradients
	at each iteration. For \rbyz, we randomly select an aggregator from 
	the pool of 64 aggregators at each iteration.}
    % trained from random initialization until convergence
    \label{fig:cifarIID}
\end{figure}

==> sections/fig_mnist_iid.tex <==

\begin{figure}[t]
\centering
    \includegraphics[width=.9\linewidth]{figs/mnist-stochastic-lr-0dot001-reverse-0dot1-bs-50/Vacc-li.pdf}\\
    % \includegraphics[width=.49\textwidth]{figures/imagenet_last/loss.pdf}
    % \hfill
    \includegraphics[width=.9\linewidth]{figs/mnist-stochastic-lr-0dot001-reverse-10-bs-50/Vacc-li.pdf}
%    \hfill
%    \includegraphics[width=.32\textwidth]{figures/cifar10_gvar/est_nvar.pdf}
    \caption{Test accuracy on MNIST with $\epsilon=0.1$ (top) and 
    $\epsilon=10$ (bottom) for the tailored attack, which is applied at each iteration.
    The total number of workers and the number of Byzantines are set to  $\nAll=12$ and $\nByz=2$, respectively.
    The dataset is randomly and equally partitioned among workers. 
	The omniscient aggregator receives and averages 10 honest gradients
	at each iteration. For \rbyz, we randomly select an aggregator from 
	the pool of 64 aggregators at each iteration.}
    % trained from random initialization until convergence
    \label{fig:mnistIID}
\end{figure}


==> sections/fig_mnist_noniid.tex <==
\begin{figure}[t]
\centering
    \includegraphics[width=0.5\textwidth]{figs_neurips/mnist-h-stochastic-lr-0.001-reverse-0.1-bs-50-nb-2-rs-3/Vacc-li}
    \caption{
    \textbf{Test accuracy on MNIST under non-iid setting.}
    MixTailor is robust to Byzantine workers in the
    heterogeneous setting ($\epsilon=0.1$).
    The dataset is partitioned by labels such that each worker holds samples for a single digit.  The rest of the setup is similar to Fig.~\ref{fig:iid}.
    }
    \label{fig:mnistnonIID}
\end{figure}

%\begin{wrapfigure}{R}{0.25\textwidth}
%\vspace*{-12pt}
%    \includegraphics[width=0.25\textwidth]{figs_neurips/mnist-h-stochastic-lr-0.001-reverse-0.1-bs-50-nb-2-rs-3/Vacc-li}
%    \caption{
%    \textbf{Test accuracy on MNIST under non-iid setting.}
%    MixTailor is robust to Byzantine workers in the
%    heterogeneous setting ($\epsilon=0.1$).
%    The dataset is partitioned by labels such that each worker holds samples for a single digit.  The rest of the setup is similar to Fig.~\ref{fig:iid}.
%    }
%    \label{fig:mnistnonIID}
%\end{wrapfigure}



%\begin{wrapfigure}[13]{r}{0.5\textwidth}
%\vspace*{-12pt}
%\begin{subfigure}[l]{\linewidth}
%    \includegraphics[width=0.8\textwidth]{figs_neurips/mnist-h-stochastic-lr-0.001-reverse-0.1-bs-50-nb-2-rs-3/Vacc-li}
%\end{subfigure}
%    \caption{
%    \textbf{Test accuracy on MNIST under non-iid setting.}
%    MixTailor is robust to Byzantine workers in the
%    heterogeneous setting ($\epsilon=0.1$).
%    The dataset is partitioned by labels such that each worker holds samples for a single digit.  The rest of the setup is similar to Fig.~\ref{fig:iid}.
%    }
%    \label{fig:mnistnonIID}
%\end{wrapfigure}


%\begin{figure}[t]
%\centering
%    \includegraphics[width=\linewidth]{figs/vacc-lo-resample}
%    \caption{Test accuracy on MNIST with 
%    $\epsilon=0.1$ attack, which is applied at each iteration.
%    The total number of workers and the number of Byzantines are set to  $\nAll=12$ and $\nByz=2$, respectively.
%    The dataset is partitioned by labels such that each worker holds samples
%    for a single digit.  The omniscient aggregator receives and averages 10
%    honest gradients at each iteration. For \rbyz, we randomly select an
%    aggregator from  the pool of 64 aggregators at each iteration.}
%    \label{fig:mnistnonIID}
%\end{figure}

